Vision-centric Token Compression in Large Language Model

Real-world applications are stretching context windows to hundreds of thousand of tokens while Large Language Models (LLMs) swell from billions to trillions of parameters. This dual expansion send compute and memory costs skyrocketing, making token compression indispensable. We introduce Vision Centric Token Compression (Vist), a slow-fast compression framework that mirrors human reading: the fast path renders distant tokens into images, letting a frozen, lightweight vision encoder skim the low-salience context; the slow path feeds the proximal window into the LLM for fine-grained reasoning. A Probability-Informed Visual Enhancement (PVE) objective masks high-frequency tokens during training, steering the Resampler to concentrate on semantically rich regions-just as skilled reader gloss over function words. On eleven in-context learning benchmarks, Vist achieves the same accuracy with 2.3 times fewer tokens, cutting FLOPs by 16% and memory by 50%. This method delivers remarkable results, outperforming the strongest text encoder-based compression method CEPE by 7.6% on average over benchmarks like TriviaQA, NQ, PopQA, NLUI, and CLIN, setting a new standard for token efficiency in LLMs. The project is at https://github.com/CSU-JPG/VIST.

==> figs/random_mask.tex <==
\begin{figure}[t]
\vspace{-10pt}
    \centering   \includegraphics[width=0.48\textwidth]{figs/randommask1.pdf} 
    \vspace{-8pt}
\caption{\textbf{Impact of Frequency-based Masking on Text-Visual Semantic Distance.} Compared to model without FM, \ourname\ with FM consistently reduces the semantic distance between text token embeddings and visual features, across all masking ratios.}
\label{fig:random_mask}
\vspace{-19pt}    
\end{figure}
% Global semantic distance comparison between \ourname\ with FM and without FM across different text masking ratios on the Arxiv and Book test sets.

==> tabs/ab_encoder_len.tex <==
\begin{table}[t]
% \vspace{-8pt}
 \caption{\textbf{Ablation on the length of text inputs (in tokens) provided to the visual encoder during training}. 
% Performance is evaluated on ICL with accuracy and open-domain QA with EM.
}
\label{tab:ab_encoder_len}
% \vspace{-2pt}
\begin{center}
\begin{small}
% \renewcommand\arraystretch{1.1}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{cccccc}
    \toprule
        \textbf{Encoder} & \multicolumn{2}{c}{\textbf{ICL}} & \multicolumn{3}{c}{\textbf{Open-domain QA}}
        \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-6} 
       \textbf{Input Length}  &  {SST5} & {MR} & {TriviaQA} &{NQ} & {PopQA} \\
        \midrule
            
         
        1024 & 39.6 & 85.9 &   19.77&	6.47 &	6.63    \\
        2048 &  39.3& 73.8 &   22.85	&8.08	&9.77    \\
        4096  & \textbf{42.7} & 79.2 &   25.20 &	8.71 & 11.44  \\
        6144 & 37.8 & \textbf{90.5} &   \textbf{27.52}	& \textbf{9.24}&	\textbf{13.49}   \\
            
                
            
            \bottomrule
        \end{tabular}
}

\end{small}
\end{center}
% \vspace{-3pt}
\end{table}

==> tabs/ab_image_token_nums.tex <==
\begin{table}[t]
% \vspace{-2pt}
\caption{\textbf{The effect of visual token count for each image.} }
% \vspace{-2pt}
\label{tab:ab_token_num}
\begin{center}
\begin{small}
% \renewcommand\arraystretch{1.1}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{cccccc}
    \toprule
        \textbf{Tokens} & \multicolumn{2}{c}{\textbf{ICL}} & \multicolumn{3}{c}{\textbf{Open-domain QA}}
        \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-6} 
       \textbf{Per Image}  &  {TREC} & {MR} & {TriviaQA} &{NQ} & {PopQA} \\
    \midrule
            
         
        32 & 32.7 & 78.8 &   19.38& 7.85 &8.16 \\
        64 &  \textbf{36.5} & 79.2 &  \textbf{25.20} & \textbf{8.71} & \textbf{11.44}     \\
        96 & 32.0 & 79.7 &    14.57&	7.19	& 4.88 \\
        128 & 32.9 & \textbf{87.0} &  20.01 &7.77 &8.51   \\

    \bottomrule
        \end{tabular}
}
% \vspace{-14pt}
\end{small}
\end{center}
\end{table}

==> tabs/ab_strategy.tex <==
\begin{table}[t]
% \vspace{-8pt}
\caption{\textbf{The effect of different masking strategies in PVE (\S\ref{sec::FCL}).} FM stands for frequency-based masking strategy. RM is short for random masking strategy. The masking ratio is set to 50\%. 
% We report accuracy for ICL tasks and EM score for open-domain QA.
}
\label{tab:ab_strategy}
% \vspace{-2pt}
\begin{center}
\begin{small}
% \renewcommand\arraystretch{1.1}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{cccccccc}
    \toprule
        &   & \multicolumn{2}{c}{\textbf{ICL}} & \multicolumn{3}{c}{\textbf{Open-domain QA}}
        \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-7} 
        \multicolumn{1}{c}{\multirow{-2}{*}{\hspace{0.5mm}\textbf{FM}   \hspace{0.5mm}}}    & \multicolumn{1}{c}{\multirow{-2}{*}{\hspace{0.5mm}\textbf{RM}   \hspace{0.5mm}}}  &  {SST5} & {MR} & {TriviaQA} &{NQ} & {PopQA} \\
        \midrule
            
            &   & 34.5 & 77.3 & 17.14 & 6.51 & 5.72	 \\
            \cmark &  & \bf42.7 & \textbf{79.2} &  \textbf{25.20} & \textbf{8.71} & \textbf{11.44} \\
             &  \cmark &  40.5 & 76.2 & 24.88 & 8.35 & 10.19	  \\
            
                
            
            \bottomrule
        \end{tabular}
}

\end{small}
\end{center}
% \vspace{-20pt}
\end{table}

==> tabs/ablation_all_icl.tex <==

\begin{table*}[t] % 使用 table* 环境支持跨双栏
\caption{\textbf{The effect of different masking strategies in Probability-Informed Visual Enhancement on In-context learning}. We report the accuracy averaged across 3 seeds (42, 43 and 44). All methods use 2 demonstrations in the decoder and 18 demonstrations in the encoder. FM denotes Frequency-based Masking strategy, while RM is random masking strategy. The masking ratio is 50\%.}
\label{tab:app_icl_masking}
% \vskip 0.15in
\begin{center}
% \begin{small}
% \setlength\tabcolsep{3.5pt}
\renewcommand\arraystretch{1.2}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{cccccccccccccc}
    \toprule
     \textbf{FM} & \textbf{RM}  & \textbf{SST2} & \textbf{MR} & \textbf{AGN} & \textbf{SST5} & \textbf{NLUS} & \textbf{NLUI} & \textbf{TREC} & \textbf{TREF} & \textbf{DBP} & \textbf{BANK} & \textbf{CLIN} & \textbf{Avg.} \\
\midrule
   & & 70.1 & 77.3&55.3	&34.5&	9.9&	26.4&	36.3&	11.2&	61.3&	15.2	&42.8&	40.0\\
    
    & \cmark &  72.8&	76.2&	60.1	&40.5	&8.3	&30.2	&32.6 &	13.3&	66.0	&20.1&	38.9&	41.7\\
    
    \cmark &   & \bf77.7 &	\bf79.2 &	\bf61.5 &	\bf42.7 &	\bf15.6 &	\bf40.6 &	\bf36.5 &	\bf14.6 &	71.9 &	25.0 &	\bf43.8 &	\bf46.3 \\

    
    \bottomrule
    \end{tabular}
    }
% \end{small}
\end{center}
\end{table*}

\begin{table*}[t] % 使用 table* 环境支持跨双栏
\caption{\textbf{The effect of different visual token count for each image on In-context learning}. We report the accuracy averaged across 3 seeds (42, 43 and 44). All methods use 2 demonstrations in the decoder and 18 demonstrations in the encoder.}
\label{tab:app_icl_token_num}
% \vskip 0.15in
\begin{center}
% \begin{small}
% \setlength\tabcolsep{3.5pt}
\renewcommand\arraystretch{1.2}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{ccccccccccccc}
    \toprule
     \textbf{Tokens Per Image} & \textbf{SST2} & \textbf{MR} & \textbf{AGN} & \textbf{SST5} & \textbf{NLUS} & \textbf{NLUI} & \textbf{TREC} & \textbf{TREF} & \textbf{DBP} & \textbf{BANK} & \textbf{CLIN} & \textbf{Avg.} \\
\midrule
     32& 85.7&	78.8	&\bf63.5&	38.0	&11.3	&27.1	&32.7&	12.0	&\bf73.4&	22.1&	40.6 & 44.1 \\
     
     64 & 77.7 &	79.2 &	61.5 &	\bf42.7 &	\bf15.6 &	\bf40.6 &	\bf36.5 &	\bf14.6 &	71.9 &	\bf25.0 &	\bf43.8 &	\bf46.3 \\
     
      96& 83.9&	79.7	&58.6	&37.0	&9.6&	29.7&	32.0&	11.5	&69.1	&20.6	&37.1	&42.6 \\
      
      128& \bf89.6&	\bf87.0&	60.3&	39.6	&11.2&	29.4	&32.9	&13.3	&70.4&	25.1&	39.8 & 45.3 \\

    
    \bottomrule
    \end{tabular}
}
% \end{small}
\end{center}
\end{table*}


\begin{table*}[t] % 使用 table* 环境支持跨双栏
\caption{\textbf{The effect of the length of text inputs (in tokens) provided to the visual encoder during training}. We report the accuracy averaged across 3 seeds (42, 43 and 44). All methods use 2 demonstrations in the decoder and 18 demonstrations in the encoder. }
\label{tab:app_icl_input_len}
% \vskip 0.15in
\begin{center}
% \begin{small}
% \setlength\tabcolsep{3.5pt}
\renewcommand\arraystretch{1.2}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{ccccccccccccc}
    \toprule
     \textbf{Encodr Input Length} & \textbf{SST2} & \textbf{MR} & \textbf{AGN} & \textbf{SST5} & \textbf{NLUS} & \textbf{NLUI} & \textbf{TREC} & \textbf{TREF} & \textbf{DBP} & \textbf{BANK} & \textbf{CLIN} & \textbf{Avg.} \\
\midrule
     1024& 77.6	&85.9	& \bf63.4	&39.6	&12.2	&32.9&	35.3	&13.9&	66.1&	\bf27.1	&42.4	&45.1  \\
     
     2048 & 78.8	&73.8	&61.6	&39.3	&12.9	&34.2&	35.8&	13.7	&67.4&	26.3&	\bf44.8	&44.4\\
     
      4096& 77.7 &	79.2 &	61.5 &	\bf42.7 &	\bf15.6 &	\bf40.6 &	\bf36.5 &	\bf14.6 &	\bf71.9 &	25.0 &	43.8 &	\bf46.3 \\
      
      6144& \bf81.7	& \bf90.5	&63.2	&37.8&	11.3	&32.6	&34.4	&13.2&	68.8&	24.7	&42.2&	45.5 \\

    
    \bottomrule
    \end{tabular}
}
% \end{small}
\end{center}
\end{table*}

==> tabs/empty_tokens.tex <==

\begin{table*}[t] % 使用 table* 环境支持跨双栏
\caption{\textbf{The impact of masking empty tokens on In-context Learning} (ICL). ICL accuracy averaged across 3 seeds (42, 43 and 44).
\ourname* does not mask attention to the empty white patches after the end of the text sequence.
\ourname* and \ourname\ use 2 demonstrations in the decoder, and the remaining demonstrations to the encoder. 
}
\label{tab:empty_tokens}
% \vskip 0.15in
\begin{center}
% \begin{small}
% \setlength\tabcolsep{3.5pt}
\renewcommand\arraystretch{1.2}
\resizebox{.99\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
    \toprule
     \textbf{Method}  & \textbf{SST2} & \textbf{MR} & \textbf{AGN} & \textbf{SST5} & \textbf{NLUS} & \textbf{NLUI} & \textbf{TREC} & \textbf{TREF} & \textbf{DBP} & \textbf{BANK} & \textbf{CLIN} & \textbf{Avg.} \\
\midrule
    \textbf{Total Demonstrations $=20$} &   &  &   &   &   &   &   &   &   &   &  &  \\
\midrule
    \ourname* & 88.7&	88.9&	65.2	&36.9&	8.4&	24.8&	38.8&	11.4&	61.2	&18.0&	42.0 & 44.0 \\
    \ourname & 77.7 &	79.2 &	61.5 &	\bf42.7 &	15.6 &	\bf40.6 &	36.5 &	14.6 &	71.9 &	25.0 &	43.8 &	46.3 \\
    \bottomrule
    \end{tabular}
    }
% \end{small}
\end{center}
\end{table*}



\begin{table}[t]
\caption{\textbf{The impact of masking empty tokens on Open-domain QA.} 
\ourname* does not mask attention to the empty white patches after the end of the text sequence. $k_\text{e}$ represents the number of passages provided to the encoder, while $k_\text{d}$ denotes the number of passages given to the LLM. We report the exact match score.}
\label{table:empty_token_qa}
\begin{center}
\begin{small}
\renewcommand\arraystretch{1.1}
% \resizebox{0.48\textwidth}{!}{
\begin{tabular}{lcccccc}
            \toprule
           \textbf{Method} & $k_\text{e}$ & $k_\text{d}$ & \textbf{TriviaQA} & \textbf{NQ} & \textbf{PopQA} \\
            \midrule
            
            \ourname* & 5 & 10 & 21.82&	7.53	&8.71  \\
              \our  & 5 & 10 & \bf25.20\greenp{3.38$\uparrow$} &	\bf8.71\greenp{1.18$\uparrow$} & \bf11.44\greenp{2.73 $\uparrow$}\\
                
            
            \bottomrule
        \end{tabular}
% }

\end{small}
\end{center}
\end{table}

==> tabs/extension_llm.tex <==
\begin{table}[t]
% \vspace{-7pt}
\caption{\textbf{\ourname\ effectively reduces PPL on LCM and improves accuracy on ICL by processing additional context.} $\dagger$ means our implementation on Mistral 7B~\cite{jiang2023mistral}.}
\label{tab:extension_llm}
\begin{center}
\begin{small}
% \vspace{-10pt}
% \vspace{-12pt}
\renewcommand\arraystretch{1.1}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccccc}
    \toprule
           & \multicolumn{2}{c}{\textbf{LCM}} & \multicolumn{2}{c}{\textbf{ICL}}
        \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
       \multicolumn{1}{c}{\multirow{-2}{*}{\hspace{0.5mm}\textbf{Method}   \hspace{0.5mm}}}  &  {Arxiv} & {Book} & {SST2}  & {DBP} \\
    \midrule
         
        Mistral & 2.93 & 12.82 &   89.1 & 93.6 \\
        CEPE$^{\dagger}$ & 2.83\greenp{0.10$\downarrow$} & 12.64\greenp{0.18$\downarrow$} & 90.8\greenp{1.7$\uparrow$}  & 94.2\greenp{0.6$\uparrow$}      \\
        
        \ourname$^{\dagger}$ & \bf2.82\greenp{0.11$\downarrow$} & \bf12.61\greenp{0.21$\downarrow$} & \bf 92.8\greenp{3.7$\uparrow$}	& \bf 95.3\greenp{1.7$\uparrow$} \\
          

    \bottomrule
    \end{tabular}
}

\end{small}
\end{center}
% \vspace{-23pt}
\end{table}

==> tabs/hpparam.tex <==

\begin{table*}[hb!]
\centering

\caption{\textbf{Hyperparameters in \ourname\ pretraining.}}
\label{table:param}
\scalebox{0.9}{
\begin{tabular}{ll}
\hline
\toprule
\multicolumn{1}{l}{\multirow{-1}{*}{\textbf{Parameter}}} & \textbf{Value} \\

\midrule
\textbf{{Data}} \\
\quad Image size (height, width) & $(224, 224)$ \\
\quad Image mode & RGB \\
\quad Font & Google Noto Sans\\%  (\texttt{GoNotoCurrent}) \\
\quad Font size & $10$ \\

\textbf{{Optimization}} \\
\quad Peak learning rate & $3.0e^{-4}$\\
\quad Warmup ratio & 4\% \\
\quad Learning rate scheduler & Cosine decay~\cite{loshchilov2016sgdr}  \\
\quad Optimizer & AdamW~\cite{loshchilov2017decoupled}  \\
\quad $\beta_1$ & $0.9$ \\
\quad $\beta_2$ & $0.999$ \\
\quad $\epsilon$  & $10^{-8}$ \\
\quad Mixed precision training & \texttt{fp16} \\
\quad Number of steps & 2000 steps\\


\bottomrule
\hline
\end{tabular}
}
\end{table*}

==> tabs/rendering_strategy_ICL.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Different Rendering Strategies for 18 demonstrations.}}
\label{tab:rendering_strategies}
\renewcommand\arraystretch{1.3}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{Description} \\  
\midrule
\bf 2-Image Rendering & All 18 demonstrations rendered into 2 images (high compression). \\  
\bf 3-Image Rendering & All 18 demonstrations rendered into 3 images (balanced compression). \\  
\bf Dynamic Rendering & All demonstrations rendered into a suitable number of images based on text length. \\  
\bf Dynamic + Blank Lines & All demonstrations rendered into a suitable number of images with blank lines between demos. \\
\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[t]
\caption{\textbf{Performance of Different Rendering Strategies on In-context learning tasks.} $k_\text{e}$ represents the number of demonstrations provided to the encoder, while $k_\text{d}$ denotes the number of demonstrations given to the LLM. We report the average accuracy across three random seeds.}
\label{tab:rendering_ICL}
\begin{center}
\begin{small}
\renewcommand\arraystretch{1.3}
% \resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
            \toprule
           \textbf{Method} & $k_\text{e}$ & $k_\text{d}$ & \textbf{SST2} & \textbf{MR}  \\
            \midrule
           \bf 2-Image Rendering   & 18  & 2 &76.0 & 77.7  \\
          \bf  3-Image Rendering   & 18  & 2 & 76.6\greenp{0.6$\uparrow$} & 78.2\greenp{0.5$\uparrow$} \\
           \bf Dynamic Rendering   & 18  & 2 & 77.0\greenp{1.0$\uparrow$} & 78.4\greenp{0.7$\uparrow$} \\
           \bf Dynamic + Blank Lines   & 18  & 2&\bf 77.7\greenp{1.7$\uparrow$} & \bf79.2\greenp{1.5$\uparrow$}  \\
            
                
            
            \bottomrule
        \end{tabular}
% }

\end{small}
\end{center}
\end{table}

==> tabs/two.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/image1.png}
    \caption{Caption for the first image.}
    \label{fig:image1}
  \end{minipage}%
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/image2.png}
    \caption{Caption for the second image.}
    \label{fig:image2}
  \end{minipage}
\end{figure}

